Parallel Clique Counting and Peeling Algorithms

We present a new parallel algorithm for $k$-clique counting/listing that has polylogarithmic span (parallel time) and is work-efficient (matches the work of the best sequential algorithm) for sparse graphs. Our algorithm is based on computing low out-degree orientations, which we present new linear-work and polylogarithmic-span algorithms for computing in parallel. We also present new parallel algorithms for producing unbiased estimations of clique counts using graph sparsification. Finally, we design two new parallel work-efficient algorithms for approximating the $k$-clique densest subgraph, the first of which is a $1/k$-approximation and the second of which is a $1/(k(1+\epsilon))$-approximation and has polylogarithmic span. Our first algorithm does not have polylogarithmic span, but we prove that it solves a P-complete problem. In addition to the theoretical results, we also implement the algorithms and propose various optimizations to improve their practical performance. On a 30-core machine with two-way hyper-threading, our algorithms achieve 13.23--38.99x and 1.19--13.76x self-relative parallel speedup for $k$-clique counting and $k$-clique densest subgraph, respectively. Compared to the state-of-the-art parallel $k$-clique counting algorithms, we achieve up to 9.88x speedup, and compared to existing implementations of $k$-clique densest subgraph, we achieve up to 11.83x speedup. We are able to compute the $4$-clique counts on the largest publicly-available graph with over two hundred billion edges for the first time.

==> algorithms-figures.tex <==





==> analysis.tex <==
\section{\framework Algorithms}\label{sec-alg}


==> app.tex <==


\section{Parallel Fibonacci heap}\label{sec-fib}
Fibonacci heaps were first introduced by Fredman and
Tarjan~\cite{FrTa84}. 
In this section, we show that we can parallelize batches of insertion
and decrease-key operations work-efficiently, with logarithmic
span. Also, we show that a single work-efficient parallel delete-min can
be performed with logarithmic span, which is sufficient for our purposes.

Previous work has also explored parallelism in Fibonacci heaps.
Driscoll et al.~\cite{DrGaShTa88} present relaxed heaps, which achieve
the same bounds as Fibonacci heaps, but can be used to obtain a
parallel implementation of Dijkstra's algorithm; however their data
structures do not support batch-parallel insertions or decrease-key
operations.  Huang and Weihl~\cite{Huang1991} and
Bhattarai~\cite{Bhattarai2018} present implementations of parallel
Fibonacci heaps by relaxing the semantics of delete-min, although no
theoretical bounds are given.



%% and there has been previous work on parallel and
%% concurrent algorithms for binary heaps and Fibonacci
%% heaps~\cite{BiBr87, DrGaShTa88, Huang1991}; however, the primary focus
%% of these works is using relaxations or locks to allow for delete-min
%% operations to occur in parallel with other operations.

%% For our purposes, we can perform each delete-min operation separately and
%% we need only parallelize batches of insert and decrease-key
%% operations. We introduce here rigorous parallel bounds for a
%% batch-parallel Fibonacci heap.

A \defn{Fibonacci heap} $H$ consists of heap-ordered trees (maintained
using a root list), with certain nodes marked and a pointer to the
minimum element. Since we use $H$ to bucket values with the same key, each node consists of a key and an associated bucket, which holds a list of the values. 
Let $n$ denote the number of elements in our
Fibonacci heap. The \defn{rank} of a node $x$ is the number of
children that $x$ contains, and the \defn{rank} of a heap is the
maximum rank of any node in the heap. Note that the rank of a
Fibonacci heap is bounded by $\BigO{\log n}$. We also define $t(H)$ to
be the number of trees in $H$, and we define $m(H)$ to be the number
of marked nodes in $H$.

We begin by giving a brief overview of the sequential Fibonacci heap operations:
\begin{itemize}
\item \textbf{Insert} ($\BigO{1}$ work): To insert node $x$, we add $x$ to the root list as a new singleton tree and update the minimum pointer if needed.
\item  \textbf{Delete-min} ($\BigO{\log n}$ amortized work): We delete the minimum node as given by the minimum pointer, and add all of its children to the root list. We update the minimum pointer if needed. We then merge trees until no two trees have the same rank; a merge occurs by taking two trees of the same rank, and assigning the larger root as a child of the smaller root.
\item \textbf{Decrease-key} ($\BigO{1}$ amortized work): To decrease the key of a node $x$, we first check if decreasing the key would violate heap order. If not, we simply decrease the key and update the minimum pointer if needed. Otherwise, we cut the node $x$ and its subtree from its parent, and add it to the root list. If the parent of $x$ was unmarked, we mark the parent. Otherwise, we cut the parent, add it to the root list, and unmark it; we recurse in the same manner on its parent.
\end{itemize}

Note that for our amortized analysis, our potential function is $\Phi(H) = t(H) + 2 \cdot m(H)$.
\par We also make a few key modifications for our purposes. Instead of keeping marks on nodes as a boolean value, each node stores a number of marks which it accumulates. Moreover, we keep a parallel hash table that stores pointers to nodes, keyed by the keys of the nodes; we use here a parallel hash table
based on linear probing~\cite{ShBl14}. The added hash table is necessary to ensure that all nodes with the same key are aggregated into a single node.

\subsection{Batch insertion}\label{sec-batch-insert}
For parallel batch insertion, let $K$ denote the set of key value pairs that we are adding to our heap. First, we semisort the keys in $K$. For each distinct key, we then check if it appears in our hash table; if so, then we simply add the corresponding set of values to the existing bucket in the heap as a batch. Otherwise, we add the new key to the hash table, and create a singleton tree where the bucket consists of all new values corresponding to that key. We add all new singleton trees to the root list, and update the minimum pointer.
\par Note that we can perform the semisort and the find operations in our hash table in parallel, in expected $\BigO{k}$ work and $\BigO{\log n}$ span w.h.p. Creating new singleton trees takes $\BigO{k}$ work and constant span, and to update the minimum pointer, we use a parallel scan between the newly added nodes and the previous minimum of the heap, which takes $\BigO{k}$ work and $\BigO{\log k}$ span.
\par The total complexity of batch insertion is given as follows.
\begin{lemma}
Parallel batch insertion of $k$ elements into a Fibonacci heap takes $\BigO{k}$ expected work and $\BigO{\log n}$ span w.h.p.
\end{lemma}

\subsection{Delete-min}
\begin{algorithm}[!t]
\caption{Parallel delete-min}
 \begin{algorithmic}[1]
\Procedure{PAR-DELETE-MIN}{$H$}
%\State Use \algname{prefix-sum} to compute a function $I$ that maps wedges to indices in order
\State Delete the minimum node and add all children to root list
\State Initialize $B$ such that $B[i]$ contains all roots with rank $i$
\While{$\exists$ a bucket in $B$ with $>1$ root}
  \State Initialize $B'$ to hold updated trees
  \ParFor{$i \leftarrow 0$ to $|B|$}
      \State Partition the roots in $B[i]$ into pairs
      \State If a root is leftover, insert it into $B'[i]$
      \State Merge the trees in every pair and insert the new roots into $B'[i+1]$
  \EndParFor
\State $B \leftarrow B'$
\EndWhile
\State Use \algname{scan} among the root nodes to update the minimum pointer
\State \Return $H$
\EndProcedure
 \end{algorithmic}
 %\caption{}
 \label{alg-delete}
\end{algorithm}

The amortized work of delete-min is $\BigO{\log n}$, but we describe how to parallelize delete-min in order to get worst-case bounds for the span.
The parallel delete-min operation is given in \algname{par-delete-min}
(Algorithm~\ref{alg-delete}). We first delete the minimum node and add
all of its children to the root list, in parallel (Line 2). Then, the
main component of our parallel delete-min operation involves consolidating
trees such that no two trees share the same rank (Lines 3--10).

In more detail, we place each tree into a bucket based on its rank
(Line 3), and then merge pairs of trees with the same rank in every
round (Lines 7--9). After $\BigO{\log n}$ rounds, each bucket will
necessarily contain at most one tree; we can show this inductively.

If we assume that after round $i$, all buckets $\leq i$ each contain
at most one tree, we see that when we process round $i+1$, no merged
tree can be added to an bucket $\leq i+1$ (since the rank of merged
trees can only increase). Moreover, bucket $i+1$ contains at most one
leftover root, and all other roots have been merged and inserted into
bucket $i+2$. Thus, the number of rounds needed to complete our
consolidation step is bounded above by the rank of $H$, which is
$\BigO{\log n}$.

The final step in our algorithm is updating the minimum pointer (Line
11).

The amortized work of our parallel delete-min operation is precisely
the amortized work of the sequential delete-min operation. This is
because the actual cost of our parallel delete-min operation is
precisely the actual cost of the sequential delete-min operation, and
the amortized analysis follows directly. Our actual cost is given by
$\BigO{t(H)+\log n}$, where $t(H)$ accounts for merging trees and
$\log n$ accounts for adding the children of the minimum node to the
root list and updating the minimum pointer. Moreover, if we let $H'$
represent our heap after performing \algname{par-delete-min}, the
change in potential is $\Delta \Phi \leq \allowbreak t(H') - t(H) \leq
\allowbreak \text{rank}(H') +1 - t(H) = \allowbreak \BigO{\log n -
  t(H)}$, because no two trees have the same rank after performing our
consolidations. Thus, in total, the amortized work is $\BigO{\log n}$,
as desired.


\begin{algorithm}[t!]
\caption{Parallel batch decrease-key}
 \begin{algorithmic}[1]
\Procedure{BATCH-DECREASE-KEY}{$H$, $K$}
\State \Comment $K$ is an array of triples, holding the key-value pair to be decreased and the updated key
\State Let $n_k$ be $\#$ times $k$ appears in a key-value pair in $K$
\State Initialize $I$ to be an array of key-value pairs that must be re-inserted
\State Initialize $K'$ to be an updated $K$
\ParFor{$(k,v,k') \in K$}
  \If{$n_k=$ size of $k$'s bucket and $v$ is the first element in the bucket}
        \State Add $(k,v,k')$ to $K'$
      \Else
         \State Add $(k',v)$ to $I$ and remove $v$ from the bucket
     \EndIf
\EndParFor
\State Initialize $M$ to be an array of marked nodes
\ParFor{$(k,\_, k') \in K'$}
  \If{changing the key to $k'$ violates heap order}
    \State Cut $k$ and add to root list with key $k'$
    \State Add a mark to the original parent of $k$ and add the parent to $M$
  \Else
    \State Change the key to $k'$
  \EndIf
\EndParFor
 \State $M\leftarrow $ nodes in $M$ with $>1$ marks
\While{$M$ is nonempty}
  \State Initialize $M'$ to be an array of marked nodes
  \ParFor{$p \in M$}
    \State Cut $p$ and add to root list
    \State Set $\#$ marks on $p$ to $0$ if $\#$ marks on $p$ is even, and $1$ otherwise
    \State Add a mark to $p$'s original parent and add the parent to $M'$
  \EndParFor
 \State $M\leftarrow$ nodes in $M'$ with $>1$ marks
\EndWhile
\State $H\leftarrow $ \algname{batch-insert}($I$)
\State \Return $H$
\EndProcedure
 \end{algorithmic}
 %\caption{}
 \label{alg-decrease}
\end{algorithm}

The span of our algorithm is dominated by the span of the while
loop. In particular, note that every iteration of our while loop has
$\BigO{1}$ span, because we can perform the pairwise merges fully in
parallel. As we previously discussed, we have at most $\BigO{\log n}$
iterations of our while loop, and so the span of parallel delete-min is
$\BigO{\log n}$. The total complexity of parallel delete-min is as
follows.

\begin{lemma}
Parallel delete-min for a Fibonacci heap takes $\BigO{\log n}$
amortized work and $\BigO{\log n}$ worst-case span.
\end{lemma}


\subsection{Batch decrease-key}
The parallel batch decrease-key operation is given in
\algname{batch-decrease-key} (Algorithm~\ref{alg-decrease}). 
We first ascertain if a node needs to be decreased. If not all values in the bucket need to be updated, then those values can simply be removed and reinserted with the updated key; the bucket holding the rest of the values can remain with the original key. Otherwise, if all values in the bucket need to be updated, we keep only the first element in the bucket and  decrease the key for that element, and we reinsert the other values with the updated key (Lines 3--10). Note that for all key-value pairs that must be reinserted, we perform all insertions in batch on Line 26, using the algorithm in Section \ref{sec-batch-insert}.
\par Note that we can determine if all values in a bucket need to be updated by using a parallel hash table to aggregate counts on the number of times each key appears in $K$. This takes $\BigO{k}$ work and $\BigO{\log k}$ span. Moreover, as discussed in Section \ref{sec-batch-insert}, our batch insertions take $\BigO{k}$ work and $\BigO{\log n}$ span w.h.p.

\par We consider for the rest of this section the nodes whose keys must actually be decreased. We check if these decreases
violate heap order (Line 13). If not, we can directly decrease the key (Line 17). Otherwise, we cut these nodes from their
trees and mark their parents (Lines 14--15). Then, we recursively cut
all parents that have been marked more than once, mark their parents,
and repeat (Lines 18--25).
\par Note that on Lines 15 and 24, we increment the number of marks of nodes in parallel, which could cause conflicts if the same parent node must be marked multiple times. Instead, to obtain our complexity bounds, we can record in an array when we would like to mark a parent. Then, we can semisort the array and use reduce to obtain the number of marks to be added to each parent. This maintains our work bounds, but note that the span of the semisort is $\BigO{\log n}$ w.h.p.

We now focus on the amortized work analysis. Let $k$ denote the
number of keys in $K$ and let $c$ be the total number of cuts that we
perform in this algorithm. Note that decreasing our keys takes
$\BigO{k}$ total work, and the rest of the work is given by the total
number of cuts, or $\BigO{c}$.

Recall that our potential function is $\Phi(H) = t(H) + 2 \cdot
m(H)$. Let $H'$ represent our heap after performing
\algname{batch-decrease-key}. The change in the number of trees is
given by $t(H') - t(H) = c$, since every new cut produces a new tree.

The change in the number of marks is $m(H') - m(H) \leq k-(c-k) =
2k - c$. The argument for this is similar to the sequential
argument.

For each cut parent node $p$, we arbitrarily set a key in $K$ as having 
\emph{propagated} the cut as follows. Let $c(p)$ denote the key that propagated the cut parent $p$, and let $M(p)$ denote the set of all nodes that marked $p$ in the round immediately before $p$ was cut. Then, we set $c(x) = x$ for each key $x$ in $K$, and we set $c(p)$ to be an arbitrary key in $C(p) = \{ c(p') \mid p' \in M(p) \}$; in other words, $c(p)$ is one of the keys that propagated a node that marked $p$ in the round immediately before $p$ was cut.

Each key $x$ then has a well-defined \emph{propagation path}, which is the maximal path of nodes that $x$ has propagated. The last node $\ell$ of the propagation path must either be a root node or a node whose parent $x$ has not propagated. Note that $x$ may mark $\ell$'s parent without cutting this parent from its tree; we call this mark an \emph{allowance}. In this sense, each key $x$ in $K$ has one mark in its allowance. We have $k$ marks in the total allowance of our heap.

It remains, then, to count the change in the number of marks on each propagation path. We claim that if we have already counted the $k$ allowances in the change in the number of marks $(m(H') - m(H) )$, we can now subtract a mark for each cut parent on a propagation path. There are two cases.

If a cut parent $p$ at the start of our algorithm already contained a
mark, then the node that propagated the cut added a mark, canceling
out the previous mark. Thus, $c(p)$ has effectively subtracted a mark
from $p$.

If a cut parent $p$ had no marks at the start of our algorithm, a
child node $p'$ such that $c(p') \neq c(p)$ must have marked $p$
within our algorithm. Necessarily, $c(p')$ must have ended its
propagation path at $p'$, so it charged its mark allowance to
$p$. Then, when the node that propagated the cut, $c(p)$, added a
mark, this cancels out the mark that $p'$ made. Since we have already
counted the mark that $p'$ made in its allowance, we can subtract a
mark to account for the cancellation.

In total, we see that we can subtract a mark for each cut parent on a
propagation path. The number of cut parents is at least $c-k$, so we
have $m(H') - m(H) \leq k - (c-k) = 2k-c$, as desired.

As such, the change in potential is $\Phi(H')-\Phi(H) \leq c + 2(2k-c)
= 4k - c$.  The actual work of \algname{batch-decrease-key} is
$\BigO{k+c}$, and the amortized work of is $\BigO{k+c} +
4k-c=\BigO{k}$ by scaling up the units of potential appropriately.

The span of our algorithm is again dominated by the span of the while
loop. We have at most $\BigO{\log n}$ iterations of the while loop,
since it is bounded by the maximum tree height of our heap, which is
bounded by the rank of the heap. Each iteration of the while loop has span $\BigO{\log n}$, due to the semisort needed to accumulate marks. Thus, the span of our algorithm is $\BigO{\log^2 n}$.

The total complexity of parallel
batch decrease-key is as follows.

%TODO the first mark on a node is part of the k allowance; the second mark on the node makes the cut and counts for -c
%TODO c + 2*2k - 2c = 4k-c
\begin{lemma}
Parallel batch decrease-key of $k$ elements into a Fibonacci heap
takes $\BigO{k}$ amortized work and $\BigO{\log^2 n}$ span.
\end{lemma}



% for insert -- insert all nodes as singletons in parallel (span 1, work n), and use a parallel scan to find the minimum between the singleton nodes and the previous min of the tree (span log n, work n)
% for delete -- put into buckets; if we have B trees of rank d, we merge into floor(b/2) trees of rank d+1; each merge is O(1) and O(1) depth trivially, since it's just re-linking; we'd have to repeat max log n rounds (max rank rounds)
% for decrease key -- first go through and decrease all keys (no cuts); then, for every key we decreased, check if it violates heap order; if it does, cut and put into the root list; also, mark parent
%    we save a list of all marked parents; then, in each round, if parent has been marked multiple times, we cut it, put into root list, save list of its parents, repeat
%    max num of rounds is max depth of a tree in our fibonacci heap, which is max rank, which is log n
%   at v end remember to update min pointer in the samee way we did with insert





==> approx.tex <==
\subsection{Approximate counting}\label{sec:approx-count}
Sanei-Mehri \textit{et al.}~\cite{SaSaTi18} describe for computing
approximate total butterfly counts based on sampling and graph
sparsification.  Their sparsification methods are shown to have better
performance, and so we focus on parallelizing these methods.  The
methods are based on creating a sparsified graph, running an exact
counting algorithm on the sparsified graph, and scaling up the count
returned to obtain an unbiased estimate of the total butterfly
count. 

The \defn{edge sparsification} method sparsifies the graph by keeping
each edge independently with probability $p$. The butterfly count of
the sparsified graph is divided by $p^4$ so obtain an unbiased
estimate (since each butterfly remains in the sparsified graph with
probability $p^4$. Our parallel algorithm simply applies a filter over
the adjacency lists of the graph, keeping an edge with probability
$p$. This takes $\BigO{m}$ work and $O\BigO{\log m}$ span.

The \defn{colorful sparsification} method sparsifies the graph by
assigning a random color in $[1,\ldots,\lceil 1/p \rceil]$ to each
vertex and keeping an edge if the colors of its two endpoints
match. Sanei-Mehri \textit{et al.}~\cite{SaSaTi18} show that each
butterfly is kept with probability $p^3$, and so the butterfly count
on the sparsified graph is divided by $p^3$ to obtain an unbiased
estimate.  Our parallel algorithm uses a hash function to map each
vertex to a color, and then applies a filter over the adjacency lists
of the graph, keeping an edge if its two endpoints have the same
color. This takes $\BigO{m}$ work and $O\BigO{\log m}$ span.

The variance bounds of our estimates are the same as shown by
Sanei-Mehri \textit{et al.}~\cite{SaSaTi18}, and we refer the reader
to their paper for details.  The expected number of edges in both
methods is $pm$, and by plugging this into the bounds for exact
butterfly counting, and including the cost of sparsification, we
obtain the following theorem.

\begin{theorem}
Approximate butterfly counting with sampling rate $p$ can be performed
in $\BigO{(1+\alpha' p) m}$ expected work and $\BigO{\log m}$ span
w.h.p., where $\alpha'$ is the arboricity of the sparsified graph.
\end{theorem}


==> figure_overview.tex <==
\begin{figure*}[!t]
  \centering
    \includegraphics[width=\textwidth]{images/clique-counting.pdf}
    \caption{Overview of our approach.}\label{fig:clique_counting}
\end{figure*}


==> figures.tex <==
%% \section*{Figure Pages}
%% These pages contain only figures.




==> framework.tex <==
\section{\framework Framework}\label{sec-framework}
In this section, we describe the \framework framework and its
components. Section~\ref{sec-count-framework} describes the procedures
for counting butterflies and Section~\ref{sec-framework-peel}
describes the butterfly peeling procedures.  Section~\ref{sec-alg}
goes into more detail on the parallel algorithms that can be plugged
into the framework, as well as their theoretical bounds.

\subsection{Counting Framework}\label{sec-count-framework}



\begin{figure}[!t]
\footnotesize
\begin{tcolorbox}
  \textbf{\underline{\framework Framework for Counting}}
  \vspace{0.5\baselineskip}
  \begin{enumerate}[label=(\textbf{\arabic*}),topsep=1pt,itemsep=0pt,parsep=0pt,leftmargin=10pt]
  \item  \emph{Rank vertices}: Assign a global ordering, $\text{rank}$, to the vertices.
\item \emph{Retrieve wedges}: Retrieve a list $W$ of wedges $(x,y,z)$ where $\text{rank}(y) > \text{rank}(x)$ and $\text{rank}(z) > \text{rank}(x)$.
\item \emph{Count wedges}: For every pair of vertices $(x_1,x_2)$, how many distinct wedges share $x_1$ and $x_2$ as endpoints.
\item \emph{Count butterflies}: Use the wedge counts to obtain the global butterfly count,  per-vertex butterfly counts, or per-edge butterfly counts.
\end{enumerate}
\end{tcolorbox}
\caption{\framework Framework for Counting}\label{fig:framework}
%\vspace{-10pt}
\end{figure}

\begin{figure*}[!t]
\centering
\footnotesize
\begin{tcbraster}[raster columns=4, raster valign=top,
raster force size=false,
raster equal height,
]
%\hspace{-.3cm}
\begin{tcolorbox}[width=.15\linewidth, colback=black!2!white,]
\textbf{\underline{Step 1}}
\vspace{0.4\baselineskip}
\begin{enumerate}[leftmargin=*]
\setlength{\itemsep}{1pt}
\item $v_3$
\item $u_1$
\item $u_2$
\item $v_1$
\item $v_2$
\item $u_3$
\end{enumerate}
\end{tcolorbox}
\begin{tcolorbox}[width=.23\linewidth, colback=black!2!white,]
\textbf{\underline{Step 2}}
\vspace{0.4\baselineskip}
\begin{equation*}
v_3 \begin{cases}\hspace{.2cm}  ((v_3, v_1), u_1) \\ \hspace{.2cm} ((v_3, v_2), u_1) \\ \hspace{.2cm}  ((v_3, v_1), u_2) \\ \hspace{.2cm} ((v_3,v_2),u_2) \end{cases}
\end{equation*}\vspace{0.1\baselineskip}
\begin{equation*}
u_1 \begin{cases}\hspace{.2cm} ((u_1, u_2), v_1) \\ \hspace{.2cm} ((u_1, u_2), v_2) \end{cases}
\end{equation*}
\end{tcolorbox}
\begin{tcolorbox}[width=.23\linewidth, colback=black!2!white,]
\textbf{\underline{Step 3}}
\vspace{0.4\baselineskip}
\begin{equation*}
\begin{rcases*}
 ((v_3, v_1), u_1) \hspace{.2cm} \\ ((v_3, v_1), u_2) \hspace{.2cm} \end{rcases*}\Rightarrow
\end{equation*}\vspace{0.1\baselineskip}
\begin{equation*}
\begin{rcases*}
 ((v_3, v_2), u_1) \hspace{.2cm} \\ ((v_3,v_2),u_2)\hspace{.2cm}  \end{rcases*}\Rightarrow
\end{equation*}\vspace{0.1\baselineskip}
\begin{equation*}
 \begin{rcases*} ((u_1, u_2), v_1) \hspace{.2cm} \\ ((u_1, u_2), v_2) \hspace{.2cm} \end{rcases*}\Rightarrow
\end{equation*}
\end{tcolorbox}
\begin{tcolorbox}[width=.33\linewidth, colback=black!2!white,]
\textbf{\underline{Step 4}}
\vspace{.5\baselineskip}
\\ $+ {2 \choose 2}$ butterflies on $v_1$, $v_3$ \\
$+ (2-1)$ butterflies on $u_1$, $u_2$
\vspace{1\baselineskip}
\\ $+ {2 \choose 2}$ butterflies on $v_2$, $v_3$ \\
$+ (2-1)$ butterflies on $u_1$, $u_2$
\vspace{1\baselineskip}
\\ $+ {2 \choose 2}$ butterflies on $u_1$, $u_2$ \\
$+ (2-1)$ butterflies on $v_1$, $v_2$
\end{tcolorbox}
\end{tcbraster}
\caption{We execute butterfly counting per vertex on the graph in Figure~\ref{img_butterfly}. In Step 1, we rank vertices in decreasing order of degree. In Step 2, for each vertex $v$ in order, we retrieve all wedges where $v$ is an endpoint and where the other two vertices have higher rank (the wedges are represented as $((x,z),y)$ where $x$ and $z$ are endpoints and $y$ is the center). In Step 3, we aggregate wedges by their endpoints, and this produces the butterfly counts for Step 4. Note that if we have $w$ wedges that share the same endpoint, this produces ${w \choose 2}$ butterflies for each of the two endpoints and $w-1$ butterflies for each of the centers of the $w$ wedges.
}\label{fig-count-ex}
\end{figure*}

Figure~\ref{fig:framework} shows the high-level structure of the
\framework framework. Step 1 assigns a global ordering to the
vertices, which helps reduce the overall work of the algorithm. Step 2
retrieves all the wedges in the graph, but only where the second and
third vertices of the wedge have higher rank than the first. 
Step 3 counts for every pair of vertices the number of
wedges that share those vertices as endpoints. Step 4 uses the
wedge counts to obtain global, per-vertex, or per-edge butterfly counts.  For each step, there are
several options with respect to implementation, each of which can be
independently chosen and used together. 
%% The main challenge in parallelizing butterfly counting is in choosing these options, which 
%% offer tradeoffs between work-efficiency and performance. 
Figure~\ref{fig-count-ex} shows an example of executing each of the steps. 
The options within each step of \framework are described in the rest of this section.

%% The basis of our butterfly counting algorithms involves iterating over
%% wedges of our graph $G$ and then grouping wedges by endpoints. We
%% describe these algorithms in more detail in Section~\ref{sec-alg}, but
%% essentially, our counting algorithms consist of the following three
%% steps:




%% All of the options within our counting framework (which we describe in more detail below) are as follows:
%% \begin{itemize}[topsep=1pt,itemsep=0pt,parsep=0pt,leftmargin=15pt]
%% \item \textbf{Ranking}: side order, degree order, approximate degree order, complement degeneracy order, approximate complement degeneracy order
%% \item \textbf{Wedge aggregation}: sorting, hashing, histogramming, simple batching, wedge-aware batching
%%   \begin{itemize}
%%   \item \textbf{Max wedges in memory} (for sorting, hashing, histogramming)
%%   \item \textbf{Max array size in memory} (for batching)
%%   \end{itemize}
%% \item \textbf{Butterfly aggregation}: atomic fetch-and-add, wedge aggregation
%% \item \textbf{Count format}: global, per-vertex, per-edge
%% \item \textbf{Approximate counts}: precise, edge sparsification, colorful sparsification
%% \end{itemize}

\subsubsection{Ranking}\label{sec-framework-retrieval}
The ordering of vertices when we retrieve wedges is significant since it affects the number of wedges that we process. As we
discuss in Section~\ref{sec-prelim-rank}, Sanei-Mehri \textit{et
  al.}~\cite{SaSaTi18} order all vertices from one bipartition of the
graph first, depending on which bipartition produces the least number
of wedges, giving them practical speedups in their serial
implementation. We refer to this ordering as \defn{side order}.
Chiba and Nishizeki~\cite{ChNi85} achieve a
lower work complexity for counting by ordering vertices in decreasing
order of degree, which we refer to as \defn{degree order}.

For practical speedups, we also introduce \defn{approximate degree
  order}, which orders vertices in decreasing order of the logarithm
of their degree (\defn{log-degree}). Since the ordering of vertices in many
real-world graphs have good locality, approximate degree order
preserves the locality among vertices with equal log-degree.  We show
in the full paper that butterfly counting
using approximate degree order is work-efficient.

\defn{Degeneracy order}, also known as the ordering
given by vertex coreness, is a well-studied ordering of vertices given
by repeatedly finding and removing vertices of smallest
degree~\cite{Seidman83, MaBe83}. This ordering can be obtained
serially in linear time using a $k$-core decomposition
algorithm~\cite{MaBe83}, and in parallel in linear
work by repeatedly removing (peeling) all vertices with the smallest
degree from the graph in parallel~\cite{DhBlSh17}. The span of peeling
is proportional to the number of peeling rounds needed to reduce the
graph to an empty graph.
We define \defn{complement degeneracy order} to be the ordering
given by repeatedly removing vertices of
largest degree. This mirrors the idea of decreasing order of
degree, but encapsulates more structural information about the graph.

However, using complement degeneracy order is not 
efficient. The span of finding complement
degeneracy order is limited by the number of rounds needed to reduce a
graph to an empty graph, where each round deletes all maximum degree
vertices of the graph. As such, we define \defn{approximate complement
  degeneracy order}, which repeatedly removes vertices of
largest log-degree. This reduces the number of rounds
needed and closely approximates the number of wedges that
must be processed using complement degeneracy order. We show
in the full paper that using complement degeneracy order and approximate
complement degeneracy order give the same work-efficient bounds as
using degree order. We implement both of these using the parallel bucketing structure of Dhulipala et al.~\cite{DhBlSh17}.

In total, the options for ranking are side order, degree order,
approximate degree order, complement degeneracy order, and approximate
complement degeneracy order.
%TODO table x shows the number of wedges in section eval
%TODO put in a note about rank? and the equation and everything; maybe in conclusion?

\subsubsection{Wedge aggregation}\label{sec-framework-wcount}

We obtain wedge counts by aggregating wedges by endpoints. \framework
implements fully-parallel methods for aggregation including sorting,
hashing, and histogramming, as well as a partially-parallel batching
method.

We can aggregate the wedges by semisorting key-value pairs where the
key is the two endpoints and the value is the center.  Then, all
elements with the same key are grouped together, and the size of each
group is the number of wedges shared by the two endpoints.  We
implemented this approach using parallel sample sort from the Problem
Based Benchmark Suite (PBBS)~\cite{BlGiSi10, ShBlFiGiKySiTa12} due to
its better cache-efficiency over parallel semisort.

We can also use a parallel hash table to store key-value
pairs where the key is two endpoints and the value is a count. We 
insert the endpoints of all wedges into the table with value
$1$, and sum the values on duplicate keys. The value associated with each key then represents the number of
wedges that the two endpoints share.  We use a parallel hash table
based on linear probing with an atomic addition combining function~\cite{ShBl14}.

Another option is to insert the key-value pairs into a parallel
histogramming structure which counts the number
of occurrences of each distinct key. The parallel histogramming 
structure that we use is implemented using a combination of
semisorting and hashing~\cite{DhBlSh17}.

%% For hashing, we use a
%% concurrent hash table based on linear probing~\cite{ShBl14}, and for
%% histogramming, we use a bucketing implementation from
%% Julienne~\cite{DhBlSh17}.



%% As discussed in Section
%% \ref{sec-par-prim}, parallel semisort is not cache-efficient, and in
%% fact, parallel sample sort outperforms parallel semisort in practice
%% due to its cache-friendly behavior \cite{GuShSuBl15}; as such, even
%% though parallel semisort gives us work-efficient bounds, we use
%% parallel sample sort for its practical efficiency.


Finally, in our partially-parallel batching method we process a
batch of vertices in parallel and find the wedges incident on these
vertices. Each vertex aggregates its wedges serially, using an array
large enough to contain all possible second endpoints. The
\defn{simple} setting in our framework fixes the number of vertices in a batch as a
constant based on the space available, while the \defn{wedge-aware} setting determines the
number of vertices dynamically based on the number of wedges that each
vertex processes.

In total, the options for combining wedges are sorting, hashing,
histogramming, simple batching, and wedge-aware batching.

\subsubsection{Butterfly aggregation}
There are two main methods to translate wedge counts into butterfly
counts, per-vertex or per-edge.\footnote{For total counts, butterfly counts can simply be computed and summed in parallel directly.}
%% see Step 4 from Figure \ref{fig-count-ex} for an example of computing butterfly counts per vertex, which must then be aggregated and appropriately stored.
One method is to make use of atomic adds, and add the obtained butterfly count for the given
vertex/edge directly into an array, allowing us to obtain butterfly counts without explicit re-aggregation.

The second method is to reuse the aggregation method chosen for the
wedge counting step and use sorting, hashing, or histogramming to
combine the butterfly counts per-vertex or per-edge.\footnote{Note
  that this is not feasible for partially-parallel batching, so in
  that case, the only option is to use atomic adds.}

\subsubsection{Other options}
There are a few other options for butterfly counting in
\framework. First, butterfly counts can be computed per vertex, per
edge, or in total.  For wedge aggregation methods apart from batching,
since the number of wedges can be quadratic in the size of the
original graph, it may not be possible to fit all wedges in memory at
once; a parameter in our framework takes into account the number of
wedges that can be handled in memory and processes subsets of wedges
using the chosen aggregation method until they are all
processed. Similarly, for wedge aggregation by batching, a parameter
takes into account the available space and appropriately determines
the number of vertices per batch.

\framework also implements both edge and colorful sparsification as
described by Sanei-Mehri \textit{et al.}~\cite{SaSaTi18} to obtain
approximate total butterfly counts. For approximate counting, the
sub-sampled graph is simply passed to the framework shown in
Figure~\ref{fig:framework} using any of the aggregation and ranking
choices, and the final result is scaled appropriately.  Note that this
can only be used for total counts. Due to space constraints, we
describe and analyze the sparsification algorithms in the full version
of the paper.

%% We omit a thorough discussion of the sparsification algorithms in this paper, but we present their evaluations and further discussion is in the full version of the paper.
%% and as such cannot be combined with the peeling
%% framework described in Section~\ref{sec-framework-peel}.

Finally, Wang \emph{et al.}~\cite{Wang2019} independently describe an
algorithm for butterfly counting using degree ordering, as done in
Chiba and Nishizeki~\cite{ChNi85}, and also propose a cache
optimization for wedge retrieval. Their cache optimization involves
retrieving precisely the wedges given by Chiba and Nishizeki's
algorithm, but instead of retrieving wedges by iterating through the
lower ranked endpoint (for every $v$, retrieve wedges $(v, w,u)$ where
$w, u$ have higher rank than $v$), they retrieve wedges by iterating
through the higher ranked endpoint (for every $u$, retrieve wedges
$(v, w,u)$ where $w, u$ have higher rank than $v$).  Inspired by their
work, we have augmented \framework to include this cache optimization
for all of our orderings.



%TODO chart of all options and what effect they have in terms of cache efficiency/parallelism? like in graphit paper? locality, work-efficiency, parallelism
\begin{figure}[!b]
\footnotesize
\begin{tcolorbox}
  \textbf{\underline{\framework Framework for Peeling}}
 \vspace{0.5\baselineskip}
  \begin{enumerate}[label=(\textbf{\arabic*}),topsep=1pt,itemsep=0pt,parsep=0pt,leftmargin=10pt]
  \item  \emph{Obtain butterfly counts}: Obtain per-vertex or per-edge butterfly counts from the counting framework.
  \item \emph{Peel}: Iteratively remove vertices or edges with the lowest butterfly count from the graph until an empty graph is reached.
\end{enumerate}
\end{tcolorbox}
\caption{\framework Framework for Peeling}\label{fig:peeling-framework}
%\vspace{-8pt}
\end{figure}
\subsection{Peeling Framework}\label{sec-framework-peel}
Butterfly peeling classifies induced subgraphs by the number
of butterflies that they contain. Formally, a vertex induced
subgraph is a \defn{k-tip} if it is a maximal induced subgraph such
that for a bipartition, every vertex in that bipartition is
contained in at least $k$ butterflies and every pair of vertices
in that bipartition is connected by a sequence of
butterflies. Similarly, an edge induced subgraph is a \defn{k-wing} if
it is a maximal induced subgraph such that every edge is contained
within at least $k$ butterflies and every pair of edges is connected
by a sequence of butterflies.

The \defn{tip number} of a vertex $v$ is the maximum $k$ such that
there exists a $k$-tip containing $v$, and the \defn{wing number} of
an edge $(u,v)$ is the maximum $k$ such that there exists a $k$-wing
containing $(u,v)$. \defn{Vertex peeling}, or \defn{tip
  decomposition}, involves finding all tip numbers of vertices in
a bipartition $U$, and \defn{edge peeling}, or \defn{wing
  decomposition}, involves finding all wing numbers of edges.

The sequential algorithms for vertex peeling and edge peeling involve
finding butterfly counts and in every round, removing the vertex or
edge contained within the fewest number of butterflies,
respectively. In parallel, instead of removing a single vertex or edge
per round, we remove all vertices or edges that have the minimum
number of butterflies.

%% For example, using the graph in Figure~\ref{img_butterfly} and the counting algorithm in Figure~\ref{fig-count-ex}, we see that $u_3$ is contained within 0 butterflies, and $u_1$ and $u_2$ are each contained within 3 butterflies. If we peel on the bipartition $U$, we would peel $u_3$ in our first round, and no butterfly counts would be updated. Then, we peel $u_1$ and $u_2$ simultaneously in the second round, since both have butterfly count 3. Note that the tip number of $u_3$ is $0$, while the tip numbers of $u_1$ and $u_2$ are $3$.
 

The peeling framework is shown in Figure~\ref{fig:peeling-framework},
and supports vertex peeling (tip decomposition) and edge peeling (wing
decomposition). Because it also involves iterating over wedges and
aggregating wedges by endpoint, it contains similar parameters to
those in the counting framework. However, there are a few key
differences.


First, ranking is irrelevant, because all wedges containing a peeled
vertex must be accounted for regardless of order. Also, using atomic add
operations to update butterfly counts is not work-efficient with respect to 
our peeling data structure (see Section \ref{sec-peel-alg}), so we do not have this as an option in our implementation.
Finally, vertex or edge peeling can only be performed if
the counting framework produces per-vertex or per-edge butterfly
counts, respectively.

Thus, the main parameter for the peeling framework is the choice of
method for wedge aggregation: sorting, hashing, histogramming, simple batching, or wedge-aware batching.
%% \begin{itemize}[topsep=1pt,itemsep=0pt,parsep=0pt,leftmargin=15pt]
%% \item \textbf{Wedge aggregation}: sorting, hashing, histogramming, simple batching, wedge-aware batching 
%% \end{itemize}
These are precisely the same options described in
Section~\ref{sec-framework-wcount}.
%% Our peeling framework is
%% based on the parallel implementation of $k$-core using bucketing from
%% Julienne~\cite{DhBlSh17}.


==> table-bounds.tex <==
\begin{figure*}[!h]
  \footnotesize
  %    \setlength{\tabcolsep}{1.5pt}
\centering
%\begin{table}[]
\begin{tabular}{p{5cm}lllll}
\toprule
\textbf{Problem} &  \textbf{Algorithm} & \textbf{Work}     & \textbf{Span}     & \textbf{Space}    \\ \midrule

\multirow{6}{*}{\textbf{\kc counting}} & \ourcount{} (parallel) \hspace{0.1cm} & $\BigO{m\alpha^{k-2}}$ expected & $\BigO{\log^{k-2}m}$ \whp{} & $\BigO{m+P\alpha}$ \\
& \kclist{}~\cite{Danisch18} (serial) \hspace{0.1cm}              & $\BigO{m\alpha^{k-2}}$ & -- &  $\BigO{m}$  \\
& \kclist{}~\cite{Danisch18} (parallel) \hspace{0.1cm}          & $\BigO{m\alpha^{k-2}}$ & $\BigO{\log m + 	\alpha^{k-2} }$  & $\BigO{m + P \alpha^2}$ \\ 
& \pivoter{}~\cite{Jain2020} (serial)  \hspace{0.1cm}  & $\BigO{n \alpha^2 3^{\slfrac{\alpha}{3}}}$   & -- & $\BigO{m + n}$\\
& \pivoter{}~\cite{Jain2020} (parallel)  \hspace{0.1cm}  &   $\BigO{n \alpha^2 3^{\slfrac{\alpha}{3}}}$ &   ${}^*$      &  $\BigO{P(m + n)}$\\
& \shortstack[l]{Worst-Case Optimal Join \\ \cite{Ngo2018, Mhedhbi2019, BinaryJoin19} (parallel)} \hspace{0.1cm}             &    $\BigO{m^{\slfrac{k}{2}}}$ expected &    $\BigO{\log^{k-2} m}$  \whp{}   &  $\BigO{m^{\slfrac{k}{2}}}$   \\
\hline

\multirow{3}{*}{\textbf{\kc peeling}} & \ourpeel{} (parallel) \hspace{0.1cm} & \shortstack[l]{$\BigO{m\alpha^{k-2}+ \rho_k(G)\log n}$ \\ expected amortized} & $\BigO{\rho_k(G) \log^{k-2} n}$ \whp{} & $\BigO{m+P\alpha}$\\
& \kclist{}~\cite{Danisch18} (serial) \hspace{0.1cm}       & $\BigO{n m \alpha^{k-3}}$ & -- &   $\BigO{m}$ \\
& \coreapp{}~\cite{FaYuChLaLi19} (serial) \hspace{0.1cm}     & $\BigO{n \binom{n-1}{k-1}}$& -- &  $\BigO{m}$ \\ 
\hline

\multirow{2}{*}{\textbf{Approximate \kc peeling}} & \ourapproxpeel (parallel) \hspace{0.1cm}& $\BigO{m\alpha^{k-2}}$ expected & $\BigO{\log^{k-1} n}$ \whp{}& $\BigO{m + P \alpha}$ \\
& \kclist{}~\cite{Danisch18} (serial) \hspace{0.1cm} &   $\BigO{m \alpha^{k-2} }$  & --&   $\BigO{m}$ \\ 

\end{tabular}
%\end{table}
\caption{This figure shows the complexity bounds for \kc counting and
peeling algorithms.
Algorithms prefixed by \algname{\textbf{arb}} are the new parallel \kc
counting and peeling algorithms that we design in this paper.
In the figure, $n$ is the number of vertices, $m$ is the number of
edges, and $\alpha$ is the arboricity of the graph. $P$ is the number
of processors, and $\rho_k(G)$ is defined to be the \kc peeling
complexity of $G$, or the number of rounds needed to peel the graph
where in each round, all vertices with the minimum \kc count are
peeled ($\rho_{k}(G) \leq n$).
%
%
\endgraf
For \kc counting using the worst-case optimal join algorithm, the
space bound is the space necessary for enumeration, which could
potentially be optimized for counting specifically.  \pivoter{} did
not give the span of their parallel \kc counting algorithm in their
theoretical evaluation, as indicated by the placeholder ${}^*$.
Finally, for approximate \kc peeling, \kclist{} actually reports a
work bound of $\BigO{m \alpha^{k-2} \log n}$, but as we show in
Theorem \ref{thm:approx-peeling}, the additional $\log$ factor is
unnecessary.
%
\endgraf
We have excluded from this table a comparison of the bounds for
approximate \kc counting. Our approximate \kc counting algorithm takes
$\BigO{pm\alpha^{k-2}+m}$ expected work, $\BigO{\log^{k-2}n}$ span
\whp{}, and $\BigO{m+P\alpha}$ space, given a sampling probability of
$p$. We  compare our algorithm to Bressan \textit{et al.}'s
\algname{MOTIVO} algorithm for approximate subgraph
counting~\cite{Bressan2019}; however, while Bressan \textit{et al.} do
give complexity bounds for the preprocessing step of \algname{MOTIVO}
($\BigO{\alpha^k m}$ work and $\BigO{\alpha^k n}$ space), they do not
give complexity bounds for the actual sampling. Chakaravarthy
\textit{et al.} \cite{ChKaMuPeQuSaSc16} show that the color coding
algorithm that Bressan \textit{et al.} use for sampling takes
$\BigO{2^k n^k}$ work.
} \label{table:bounds}
\end{figure*}

